Approximate Sparse Recovery: Optimizing Time and Measurements

An approximate sparse recovery system consists of parameters $k,N$, an $m$-by-$N$ measurement matrix, $\Phi$, and a decoding algorithm, $\mathcal{D}$. Given a vector, $x$, the system approximates $x$ by $\widehat x =\mathcal{D}(\Phi x)$, which must satisfy $\| \widehat x - x\|_2\le C \|x - x_k\|_2$, where $x_k$ denotes the optimal $k$-term approximation to $x$. For each vector $x$, the system must succeed with probability at least 3/4. Among the goals in designing such systems are minimizing the number $m$ of measurements and the runtime of the decoding algorithm, $\mathcal{D}$. In this paper, we give a system with $m=O(k \log(N/k))$ measurements--matching a lower bound, up to a constant factor--and decoding time $O(k\log^c N)$, matching a lower bound up to $\log(N)$ factors. We also consider the encode time (i.e., the time to multiply $\Phi$ by $x$), the time to update measurements (i.e., the time to multiply $\Phi$ by a 1-sparse $x$), and the robustness and stability of the algorithm (adding noise before and after the measurements). Our encode and update times are optimal up to $\log(N)$ factors.

==> reftheorems.tex <==

We use the following facts repeatedly, some of which proofs are easy and thus omitted.  Others are collected below.
%\begin{lemma} Suppose $a\geq 1$ and $b > 0$. If $e^{-a}<b$ then $e^{-ax}<\frac{b}{x}$ for all $x\geq 1$.
%\end{lemma}

%\begin{proof}
%Note that $f(x) = \frac{1}{b}xe^{-ax}$ is decreasing on $[1,\infty)$.
%\end{proof}

\begin{lemma} Let $X_i$ be $n$ i.i.d. binary random variables with $E(X_i)=p$. Then $\Pr(\sum X_i > \theta n) < \left(\frac{p^\theta}{\econst^p}\left(\frac{\econst}{\theta}\right)^\theta\right)^n$. %< \left(\frac{pe}{\theta}\right)^{\theta n}$.
\end{lemma}

%\begin{proof}
%The $\delta$ in Chernoff bound is $\delta = \frac{\theta}{p}-1$, it follows that $\Pr(\sum X_i > \theta n) < \left(\frac{e}{1+\delta}\right)^{np(1+\delta)} = \left(\frac{pe}{\theta}\right)^{\theta n}$.
%\end{proof}

And we need a Poisson balls-and-bins model, as in

\begin{lemma}
	\label{poissonmodel} 
	Suppose $m$ balls are thrown independently into $n$ bins and a dustbin. After a ball is dropped, the probability that it lands in the dustbin is $1-np$, and the probability in a specific bin is $p$. Then the event that $\theta n$ bins contain $h$ ($h<mp$) balls each does not happen with probability at most 
	\[ \min\left\{\frac{2  q}{1-\theta},2(\frac{q\econst}{1-\theta})^{(1-\theta)n}\right\}
	\quad\text{where $q = \frac{\econst^{-mp}(mp)^h}{h!\left(1-\frac{h}{mp}\right)}$.}
	\]
\end{lemma}
\begin{proof}
Let $k_i$ denote the number of balls in bin $i$ and $m'$ a random variable subject to Possion distribution with mean $m$. Consider the case that $m'$ balls are thrown into $n$ bins independently. Denote by $k'_i$ denote the number of balls in bin $i$. It is easy to see that $k'_i$'s are i.i.d. random variables subject to Possion distribution with mean $mp$.

Let $f$ be an arbitrary increasing function, we have
\begin{align*}
     \Expect \left[f(k'_1,\dots,k'_n)\right] &= \sum_{m' = 0}^\infty   
         \Expect\left[f(k'_1,\dots,k'_n) | \sum k'_i = m'\right] \Prob{\sum k'_i = m'}\\
    &\geq \sum_{m' = m}^\infty \Expect\left[f(k'_1,\dots,k'_n) | \sum k'_i = m\right] 
              \Prob{\sum k'_i = m'}\\
    &= \Expect\left[f(k_1,\dots,k_n) | \sum k'_i = m\right]\Prob{m'\geq m}\\
    &\geq \frac{1}{2}\Expect\left[f(k_1,\dots,k_n)\right],
\end{align*}
whence we conclude that for an event $A$ with an increasing probability in the number of balls, if $A$ has probability $p$ in the Poission case then $A$ has probability at most $2p$ in the exact case, by taking $f = \mathbf{1}_A$.

Now we take $A$ to be the event that there exists $\theta n$ bins such that each bin contains at least $h$ balls. In the Poisson case, the probability that a specific bin contains less than $h$ balls is, by \cite[Proposition 1]{Glynn19879}, at most $q = \frac{\econst^{-mp}(mp)^h}{h!\left(1-\frac{h}{mp}\right)}$. It follows from Chernoff bound and Markov inequality that the failure probability of $\theta n$ bins containing at least $h$ balls each is at most $\left\{\frac{q}{1-\theta},\left(\frac{q\econst}{1-\theta}\right)^{(1-\theta)n}\right\}$ in the Poisson case, and thus at most doubled the quantity in the exact case.
\end{proof}

